Detecting ADS-B Spoofing Attacks using Deep Neural Networks

The Automatic Dependent Surveillance-Broadcast (ADS-B) system is a key component of the Next Generation Air Transportation System (NextGen) that manages the increasingly congested airspace. It provides accurate aircraft localization and efficient air traffic management and also improves the safety of billions of current and future passengers. While the benefits of ADS-B are well known, the lack of basic security measures like encryption and authentication introduces various exploitable security vulnerabilities. One practical threat is the ADS-B spoofing attack that targets the ADS-B ground station, in which the ground-based or aircraft-based attacker manipulates the International Civil Aviation Organization (ICAO) address (a unique identifier for each aircraft) in the ADS-B messages to fake the appearance of non-existent aircraft or masquerade as a trusted aircraft. As a result, this attack can confuse the pilots or the air traffic control personnel and cause dangerous maneuvers. In this paper, we introduce SODA - a two-stage Deep Neural Network (DNN)-based spoofing detector for ADS-B that consists of a message classifier and an aircraft classifier. It allows a ground station to examine each incoming message based on the PHY-layer features (e.g., IQ samples and phases) and flag suspicious messages. Our experimental results show that SODA detects ground-based spoofing attacks with a probability of 99.34%, while having a very small false alarm rate (i.e., 0.43%). It outperforms other machine learning techniques such as XGBoost, Logistic Regression, and Support Vector Machine. It further identifies individual aircraft with an average F-score of 96.68% and an accuracy of 96.66%, with a significant improvement over the state-of-the-art detector.

==> Sections/appendices.tex <==
\newpage
\appendix

\subsection{Simulate Transmit Frequency Offset in IQ Samples}
Each ADS-B message consists of $8\mu$s preamble and $112 \mu$s data block (112 bits in total). 
There are a total of $m=120$ pulses with different time positions to encode the information to be transmitted (i.e., Manchester coding). 
Hence, the transmitted passband signal $s_p(t)$ can be represented as follows \cite{leonardi2017air, madhow2008fundamentals}:
\begin{equation}
    s_p(t) = Re[\sqrt{2} s(t) e^{j 2 \pi f_c t}]
\end{equation}
where 
\begin{equation}
    s(t) = \left[ \sum_{m=1}^{120} rect\left( \frac{t-2mT+c_mT + T/2}{T} \right) \right],
\end{equation}
is the baseband signal with a phase of zero. 
In general, we have $s(t)=s_c(t) + j s_s(t)$ and $s_p(t) = e(t) \cos (2\pi f_c t + \theta(t))$, where $e(t)=|s(t)|=\sqrt{s_c^2(t) + s_s^2(t)}$ is the envelope and $\theta(t)=\tan^{-1} \frac{s_c(t)}{s_s(t)}$ is the phase.

In order to generate IQ samples that can be transmitted by the USRP, we first sample $s(t)$ with a sampling rate of $1/T_s$ where $T_s=T/2 =0.2\mu$s and obtain $s[k]=s(kT_s)$.  
Hence, each ADS-B message is represented by $\{s[k]\}$ with a total of $240$ samples.
After that, we generate one I sample and one Q sample for each $s[k]$.
%that have the same magnitude  and a phase of zero. 
IQ samples are then stored in the binary format as interleaving unsigned bytes. 


In the presence of a transmit frequency offset $\Delta f$, the transmitted signal with the embedded Doppler shift becomes
\begin{align}
    s_p(t) &= Re[\sqrt{2} s(t) e^{j 2 \pi (f_c + \Delta f) t}] \\
    &= Re[(\sqrt{2}s(t) e^{j 2 \pi \Delta f t}) e^{j 2 \pi f_c t}].
\end{align}
Hence, in order to simulate the transmit freqeuency offset, we can introduce a phase change in the transmitted signal by multiplying each complex sample  by $e^{j 2 \pi \Delta f t}$, where $t=kT_s$. 

\subsection{Simulate Doppler Shift}
Let the baseband signal be $s(t)$ and its passband signal at a center frequency of $f_c$ be $s_p(t)=Re[\sqrt{2}s(t)e^{j2\pi f_c t}]$. 
Let their Fourier transform be $S(f)$ and $S_p(f)$, respectively. 
The relationship between $S(f)$ and $S_p(f)$ is 
\begin{equation}
    S(f) = \sqrt{2} S_p^+ (f+f_c),
\end{equation}
where $S_p^+(f)$ is the segment of $S_p(f)$ occupying positive frequencies. 

Due to the Doppler shift, the observed frequency $f_o$ is 
\begin{equation}
    f_o = \left(\frac{c+v_o}{c-v_s} \right) f = (1 + \alpha) f,
\end{equation}
where $\alpha = \frac{c+v_o}{c-v_s} - 1$. 
As a result, the observed passband signal becomes 
\begin{equation}
    S_p'(f) = S_p \left(\frac{1}{1+\alpha} f \right).
\end{equation}
Hence, we have 
\begin{align}
    s'_p(t) &= (1+\alpha) s_p((1+\alpha) t) \\
    &=(1+\alpha) Re[\sqrt{2} s((1+\alpha)t) e^{j 2\pi  f_c (1+\alpha) t}]. 
\end{align}

For example, if $s_p(t) = \cos(2\pi f_c t)$ and $f_d=(1+\alpha) f_c$, then we have $s_p'(t) = \cos(2\pi f_d t) = s_p((1+\alpha) t)$. 

Note that since the bandwidth of ADS-B signal is about 50 kHz, it can be considered as a narrowband signal, as compared to the center frequency of 1090 MHz. 
As a result, the Doppler effect essentially results in a frequency shift \cite{matz2011fundamentals}.

==> Sections/discussion.tex <==
\section{\hl{Discussion (TODO, 0.5 page)}}
\label{sec:discussion}
\begin{itemize}
    \item Are features stable over the long term?
    \item How to perform multi-class classification for 70,000 different aircrafts? \cite{strohmeier2017large}
    From multi-class classification to binary-classification
    
    \item From per-message detection to multi-message detection: if we assume attack messages carry the same ICAO address. Then by combing results of multiple messages, we can further improve the accuracy.
    Considered as attack if 3 consecutive messages are considered as attack? Decrease both $P_{fa}$ and $P_d$
    
    \item How to deal with confusion? Clustering?
    \item Features
    
    \item scalability
    
    \item what causes confusion?
\end{itemize}

==> Sections/localization.tex <==
\section{Localization}
Multilateration is not possible. 

RSSI-based distancing can be very unreliable:
\begin{itemize}
    \item Exact transmit power is unknown (at least 21 dBW, not more than 27 dBW).
    \item Transmit/receive antenna gain is unknown
    \item Accuracy of radio propagation model 
    \item RSSI range can be up to 30 dB \cite{schafer2014bringing}
\end{itemize}
